Representation Learning for Stack Overflow Posts: How Far are We?

The tremendous success of Stack Overflow has accumulated an extensive corpus of software engineering knowledge, thus motivating researchers to propose various solutions for analyzing its content.The performance of such solutions hinges significantly on the selection of representation model for Stack Overflow posts. As the volume of literature on Stack Overflow continues to burgeon, it highlights the need for a powerful Stack Overflow post representation model and drives researchers' interest in developing specialized representation models that can adeptly capture the intricacies of Stack Overflow posts. The state-of-the-art (SOTA) Stack Overflow post representation models are Post2Vec and BERTOverflow, which are built upon trendy neural networks such as convolutional neural network (CNN) and Transformer architecture (e.g., BERT). Despite their promising results, these representation methods have not been evaluated in the same experimental setting. To fill the research gap, we first empirically compare the performance of the representation models designed specifically for Stack Overflow posts (Post2Vec and BERTOverflow) in a wide range of related tasks, i.e., tag recommendation, relatedness prediction, and API recommendation. To find more suitable representation models for the posts, we further explore a diverse set of BERT-based models, including (1) general domain language models (RoBERTa and Longformer) and (2) language models built with software engineering-related textual artifacts (CodeBERT, GraphCodeBERT, and seBERT). However, it also illustrates the ``No Silver Bullet'' concept, as none of the models consistently wins against all the others. Inspired by the findings, we propose SOBERT, which employs a simple-yet-effective strategy to improve the best-performing model by continuing the pre-training phase with the textual artifact from Stack Overflow.

==> sections/background.tex <==
\section{Background}
\label{sec:background}
\subsection{BERT-based Language Models}
Language models learn to determine the probability distribution of word occurrences from the given sentences. Such models could effectively capture text semantics and use the obtained knowledge to understand new phrases, which provide a solid basis for various applications. The emergence of BERT is one of the major innovations in natural language processing (NLP) over the last decade, and it marks the beginning of a new era. BERT-based pre-trained models~\cite{bert, roberta, albert, distillbert, transformer, longformer} have achieved phenomenal performance in a wide range of NLP tasks, including sentiment analysis~\cite{bert_sentiment}, POS tagging~\cite{bert_pos}, question answering~\cite{bert_questionanswering} etc. Such models essentially inherit the architecture of the Transformer and have been extensively pre-trained on large-scale datasets, thus eliminating the process of training language models from scratch and saving a drastic amount of time and resources. 

One of the critical factors in the success of BERT-based models is the self-attention mechanism of the Transformer. The attention mechanism can be summarized as projecting a set of queries and key-value pairs to the output vectors in a dimension of $n$, where $n$ is determined by the length of the input sequence. Given the input sequence $X$, each token $x_i$ from the input is transformed into three types of vectors, which are $q_i$, $k_i$, and $v_i$, respectively. The transformation is conducted by multiplying $x_i$ with three weight matrices, i.e. ( $W(Q)$, $W(K)$, and $W(V)$) that are learned from the training. We refer to the transformed vectors as the \textit{query, key, and value} vectors, and $Q, K, V$ are matrices denoting the concatenation of all \textit{query, key, and value} vectors. The output vectors are then calculated as:
\begin{equation}
    \texttt{Attention}(Q,K,V) = \texttt{softmax} (\frac{QK^{T}}{\sqrt{d_{k}}})V
\end{equation}

Where $d_{k}$ represents the dimension of the key vectors. In a nutshell, the proposed attention mechanism scales the dot product of query with keys with $\frac{1}{\sqrt{d_k}}$, applies the softmax operation then multiplies the previous result with value vectors. 


\subsubsection{Masked Language Modeling (MLM)}
Many previous literature~\cite{bert, roberta} have demonstrated the great effectiveness of the MLM pre-training objective. 
Formally speaking, for a given data point $x = \{n\}$ where $n$ denotes a sequence of text tokens, 15\% of tokens ($m$) are randomly masked from the input sequence, and the model is to be trained to predict the masked words to complete the sentence. 

\begin{equation*}
    x^{\text{masked}} = \text{REPLACE}(x, m^w, [MASK])
\end{equation*}

The loss function of the MLM is:

\begin{equation*}
    \mathcal{L}_{MLM}(x,\theta) = \sum_{i\in m^w
} -log p^{D1}(x_i | w^{masked})
\end{equation*}


